Approximations in the homogeneous Ising model

The Ising model is important in statistical modeling and inference in many applications, however its normalizing constant, mean number of active vertices and mean spin interaction -- quantities needed in inference -- are computationally intractable. We provide accurate approximations that make it possible to numerically calculate these quantities in the homogeneous case. Simulation studies indicate good performance of our approximation formulae that are scalable and unfazed by the size (number of nodes, degree of graph) of the Markov Random Field. The practical import of our approximation formulae is illustrated in performing Bayesian inference in a functional Magnetic Resonance Imaging activation detection experiment, and also in likelihood ratio testing for anisotropy in the spatial patterns of yearly increases in pistachio tree yields.

==> approx2.tex <==
$|R_{\ell}| \leq D_1 \{( s^\bullet - s_\bullet)/\ell_2\}/ \ell_2,$
where
%$D_1 = \max_{u \in (s_\bullet, s^\bullet)} (4\ell_2^2/\sigma_r^2) \phi'( (2\ell_2 u - \mu_r)/\sigma_r)  ( 2\ell_2 u - \mu_r)/\sigma_r$ 
$D_1$ is the maximum value of the derivative of the function being evaluated.
Note that
$( s^\bullet - s_\bullet)/\ell_2\leq 1$. However, for $\ell > k$, we have
$( s^\bullet - s_\bullet)/\ell_2 \leq \ell k/(2 \ell_2) \leq c_1 k / \ell.$
Let $\mu_{\ell} = \theta + \beta\sigma_r^2/(2\ell_2).$ We have,
\begin{multline*}
\exp(-2\beta \theta \ell_2 - \beta^2 \sigma_r^2/2) D_1 = \max_u \biggl| \frac{d}{du} \biggl\{ \frac{2\ell_2}{\sigma_r} \phi( 2\ell_2( u - \mu_{\ell}) /\sigma_r)
\biggr\} \biggr|
= \max_u \biggl|  \frac{4\ell_2^2}{\sigma_r^2} \phi'( 2\ell_2( u - \mu_{\ell}) /\sigma_r)
\biggr\} \biggr| 
= \\ 
\max_u \biggl|  \frac{4\ell_2^2}{\sigma_r^2} 
\{ (2\ell_2/\sigma_r) ( u - \mu_{\ell}) \phi( 2\ell_2( u - \mu_{\ell}) /\sigma_r) \}
 \biggr|
\leq c_2 \frac{4\ell_2^2}{\sigma_r^2} 
=c_2  \frac{\ell_2^2}{2 \ell_2 \theta (1 - \theta) ( 1 - y_{n,2})} \\
\leq c_3  \theta^{-1}(1- y_{n,2})^{-1} \ell^2
\leq c_4 (n/k) (1 - y_{n,2})^{-1} \ell^2
\end{multline*} 




\begin{comment}
########################################################
Let $\psi(G_{\ell}) = \sum_{t < h} k_{th}$. We have
\begin{align*}
  \operatorname{Var}(\sum_{h=1}^{\ell} r_h | \eta )
  &= \sigma_{\ell}^2 +
  \frac{(\ell-1)(n- \ell)}{(n-1)^2}
  \bigl\{ 2 \bigl(1 + \frac{1}{n-2} \bigr)\psi( G_{\ell}) - \frac{2 \ell_2 k^2 }{n-2} \bigr\}
  \\
 & = \sigma_{\ell}^2 +  \frac{(\ell-1)(n- \ell)}{(n-1)^2(n-2)} \{ 2(n-1) \psi( G_{\ell})
 - 2 \ell_2 k^2 \}  \\
&=  \sigma_{\ell}^2 + \frac{(\ell-1)(1 - y_{n,2})}{n-1} \{ 2 \psi( G_{\ell})
  - \frac{2 \ell_2}{n-1} k^2 \}  \\
 &= \sigma_{\ell}^2 + 2\ell_2 \theta (1 - y_{n,2}) \{ 2 \frac{\psi( G_{\ell})}{\ell k}
 - \frac{\ell-1}{n-1} k \}  \\
  &= \sigma_{\ell}^2 + \frac{\sigma_{\ell}^2}{1 -\theta} \{ 2 \frac{\psi( G_{\ell})}{\ell k}
  - \frac{\ell-1}{n-1} k \}  \\
  &=  \sigma_{\ell}^2 \biggl[ 1 +  (1 -\theta)^{-1} \{ 2 \frac{\psi( G_{\ell})}{\ell k}
  - \frac{\ell-1}{n-1} k \} \biggr]. 
\end{align*}
Obviously the quantilty $\psi( G_{\ell})$ depends on each sub-graph. 
So we need to consider that they change with each sub-graph $G_{\ell}$.
Therefore, we need to take expextation in the above expression
for  $\operatorname{Var}(\sum_{h=1}^{\ell} r_h | \eta )$.


So in practice,
we replace it by an estimate. Note that the proportion of vertices that are
neighbors of a given vertex is $k/(n-1)$, so the proportion of shared neighbors
for a given couple fo vertices is about $k^2/(n-1)^2 = \theta^2$. So $k_{th}$ should be
about $n \theta^2$. This yields the estimate of  $\operatorname{Var}(\sum_{h=1}^{\ell} r_h)$
\begin{equation*}
  \hat{\sigma}_{\ell}^2 = \sigma_{\ell}^2 \biggl[ 1 +  (1 -\theta)^{-1} \{ (\ell -1)\theta\frac{n}{n-1} - (\ell-1)\theta \}
    \biggr]
  = 
  \sigma_{\ell}^2 \biggl\{ 1 +  \frac{\theta}{1 -\theta} \frac{\ell-1}{n-1} \biggr\}.
\end{equation*}
Note that $\hat{\sigma}_{\ell}^2/  \sigma_{\ell}^2 \rightarrow 1$ as $n\rightarrow \infty$.
########################################################
\end{comment}


\begin{comment}
%##########################################
An estimate of $p_d( r |\ell )$ may be obtained using a mean-field-type estimate
which assumes that the degrees are independent. In this latter case,
\begin{align}
  \tilde{p}_d( r |\ell ) &=  \sum_{r_1 + r_2 + \cdots r_{\ell} = r } \prod_{h} p_{d,m}( r_h | \ell).
  \label{eq:hyper:prob}
\end{align}
In this case, ${\cal M}_{\tilde{p}_d(\cdot|\ell)}(\beta) = \{ {\cal M}_{p_{d,m}(\cdot|\ell)}( \beta)\}^{\ell}.$
Note however, that we need to have $r=2s$. That is, we need
$ {\cal M}_{p_d(even|\ell)}(2\beta) = \sum_s \exp( 2\beta s) p_{d}( 2s | \ell) / \sum_s p_{d}( 2s | \ell)$.
We may assume that $ \sum_s p_{d}( 2s | \ell) = 1/2$.
We have
$$
  {\cal M}_{\tilde{p}_d(\cdot|\ell)}(\beta)  = \sum_{r=0}^{\ell k} \exp( \beta r)  \tilde{p}_d( r |\ell )
  = \sum_{s=0}^{\ell k/2} \exp( \beta 2s)  \tilde{p}_d( 2s |\ell ) + 
  \exp\{ \beta (2s + 1) \}  \tilde{p}_d( 2s+1 |\ell ).
$$
But
$\sum_{s} \exp\{ \beta (2s + 1) \}  \tilde{p}_d( 2s+1 |\ell )
= \exp(\beta) \sum_{s} \exp( 2\beta s )  \tilde{p}_d( 2s+1 |\ell )$
which is approximately equal to
$\exp(\beta) \sum_{s} \exp( 2\beta s )  \tilde{p}_d( 2s |\ell ).$
Therefore we estimate ${\cal M}_{p_d(even |\ell)}$ by the quantity
$ {\cal M}_{\tilde{p}_d(even|\ell)}(2\beta) = 2{\cal M}_{\tilde{p}_d(\cdot|\ell)}(\beta) /\{1 + \exp(\beta)\}.$
Noting that
\begin{align*}
  {\cal M}'_{\tilde{p}_d(even|\ell)}(\beta) &= \frac{{\cal M}'_{\tilde{p}_d(\cdot|\ell)}(\beta/2)}{1 + \exp(\beta/2)}  - \frac{\exp(\beta/2)}{\{1 + \exp(\beta/2)\}^2} {\cal M}_{\tilde{p}_d(\cdot|\ell)}(\beta/2), \\
    {\cal M}''_{\tilde{p}_d(even|\ell)}(\beta) &= 
    \frac{{\cal M}''_{\tilde{p}_d(\cdot|\ell)}(\beta/2)}{2(1 + \exp(\beta/2))}
    - \frac{\exp(\beta/2)}{\{1 + \exp(\beta/2)\}^2}  {\cal M}'_{\tilde{p}_d(\cdot|\ell)}(\beta/2) - \\
     & \qquad \qquad {\cal M}_{\tilde{p}_d(\cdot|\ell)}(\beta/2) \biggl( \frac{\exp(\beta/2)}{2\{1 + \exp(\beta/2)\}^2}
    - \frac{\exp(\beta)}{\{1 + \exp(\beta/2)\}^3} \biggr),
\end{align*}
we have that the estimated mean and variances according to this proportion estimates are,
respectively,
$$\tilde{\mu}_d = n_2\theta y y_n -(1/4) \text{\ and\ }
\tilde{\sigma}^2_d = n_2 \theta y y_n(1 - y_{n,2}) (1 - \theta)/2 -(1/16),$$
where $\theta= m/n_2 = k/(n-1)$ is the proportion of edges with respect to a complete graph,
$y = \ell/n$ is the proportion of vertices in the subgraph, and
$y_n = (\ell -1)/(n-1) = (y - n^{-1})/(1 - n^{-1})$,
$y_{n,2} = (\ell -2)/(n-2) = (y - 2n^{-1})/(1 - 2n^{-1})$.
Note that $yy_n = \ell_2/n_2$ is the proportion of edges in a complete graph of $\ell$ vertices
with respect to the complete graph with the $n$ original vertices. 
The corresponding moments associated to the proportions $p_e(\cdot|\ell)$ are, respectively,
$$\mu_e = n_2\theta y y_n,  \text{\ and \ }
\sigma_e^2 =n_2\theta y y_n (1 - y y_n)(1 - \theta_n),$$ where
$\theta_n = (\theta - n_2^{-1})/( 1 -  n_2^{-1} ) \approx \theta.$
The first moments of these distributions are very similar. However,
$\tilde{p}_d(\cdot|\ell)$ has half as much variance than $p_e(\cdot|\ell)$.
Observe that $\tilde{\sigma}_d$ is overestimating the variance associated
to $p_d(r)$, since the variables
$r_h$ are surely negatively correlated.
This signals that $p_e(\cdot|\ell)$ is too spread to be a good estimate
of the distribution of the number of edges among the subgraphs ${G}_{\ell}$.


Because under $\tilde{p}_d(\cdot |\ell)$, $r$ is the sum of $\ell$ independent random variables,
for large $\ell$, we can use the central limit theorem to argue that
$ {\cal M}_{\tilde{p}_d(\cdot|\ell)}(\beta) \approx \exp\{ 2\beta  n_2\theta y y_n
+ \beta^2 n_2 \theta y y_n(1 - y_{n,2}) (1 - \theta) \}$, and hence
${\cal M}_{\tilde{p}_d(even|\ell)}(2\beta) \approx 2\{1 + \exp(\beta)\}^{-1}
\exp[2 \beta  n_2\theta y y_n \{ 1 + (\beta/2)(1 - y_{n,2}) (1 - \theta) \} ].$
\end{comment}



In this work, we propose three estimators of the partition function. One of them is obtained by
using the estimated distribution of the edges $p_e(\cdot|\ell)$.
We refer to this estimate as the hypergeometric edge estimate
$Z_{Hyper}(\alpha, \beta)$, which is given by
$$1 + \exp( \alpha' n + \beta k n) +
+n \exp(\alpha') + 
\sum_{\ell=2}^{n-1} \binom{n}{\ell} \sum_{s=s_\bullet}^{s^\bullet} \frac{ \binom{  \ell_2  }{ s} \binom{ n_2 - \ell_2 }{ m - s} }
{ \binom{n_2}{m} }\, \exp( \alpha'\ell + 2\beta s),$$
where $s_\bullet = \max\{0, m - n_2 +\ell_2\}$, and $s^\bullet= \min\{\ell k/2, \ell_2\}$.
The second partition function estimate, is given by the CLT approximation to
${\cal M}_{\tilde{p}_d(\cdot|\ell)}(\beta)$, which we refer to as 
the Normal degree estimate 
$Z_{Normal}(\alpha, \beta)$. This is given by
$$1 + \exp( \alpha' n + \beta k n) +
+n \exp(\alpha') + 
\sum_{\ell=2}^{n-1} \binom{n}{ny} 
\frac{2\exp[ \alpha' n y + 2\beta  n_2\theta y y_n \{ 1 + (\beta/2)(1 - y_{n,2}) (1 - \theta) \} ]}{1 + \exp(\beta)}.$$
The third estimate is based on the fact that when the m.g.f. converges to a m.g.f. of a
determined distribution, the distribution function converges to the corresponding limit
distribution function.Therefore, we may suppose that for large $\ell$,
$$ p_d(r = 2s|\ell) \approx  \int_{2(s-1/2)}^{2(s+1/2)}\frac{1}{\sigma_{\ell}} \phi\bigl( (x - \mu_r)/ \sigma_{\ell} \bigr)\, dx =
 \int_{2s-1}^{2s+1} \frac{1}{\sqrt{2 \pi}\, \sigma_{\ell}} \exp\biggl\{ -\frac{1}{2}
\frac{ (x - \mu_r)^2}{\sigma_{\ell}^2} \biggr\}\, dx,$$
with $\mu_r =2n_2\theta y y_n$, and $\sigma_{\ell}^2 = 2n_2 \theta y y_n(1 - y_{n,2}) (1 - \theta).$




==> fmriapp.tex <==
\section{Application to activation detection in  fMRI experiment}
\label{application}

\subsection{Bayesian model for voxel activation}
We illustrate the use of our approximations in fully Bayesian
inference for determining activation in a
fMRI~\citep{lazar08,lindquist08} experiment. Our fMRI 
dataset is derived from images from the twelve replicated instances of a
subject alternating between rest and also alternately tapping his
right-hand and left-hand
fingers~\citep{maitraetal02,maitra09,maitra10}. 
For this illustration, we restrict attention only to the right-hand and 
the 20th slice, noting also that our derivations are general enough 
to extend to the other hand and  the three-dimensional volume.
Our data are in the 
form of $p$-values at each pixel that measure the significance of the
positivity of the linear relationship between the pixelwise observed
Blood-Oxygen-Level-Dependent (BOLD) time series response and the
expected BOLD response obtained through a convolution of the input
stimulus time-course with the Hemodynamic Response Function.
Let 
$p_{r1},p_{r2},\ldots,p_{rn}$ be the observed $p$-values in
the $r$th replication, where $n$ is the number of pixels. Let
$X_1,X_2,\ldots,X_n$ be indicator variables, with $X_i=0$ or 1
depending on whether the $i$th pixel is truly active or not. Then, we
may model $p_{ri}$, given the true state $X_i=x_i$ of the pixel
as $f(p_{ri}\mid X_i = x_i) = \{ U( p_{ri}; 0,1) \}^{1 - x_i} \,
\{b(p_{ri}; a, b)\}^{x_i}$ 
where $U( p_{ri}; 0,1)$ is the standard uniform density, and
$b(p_{ri}; a, b)$ is the density of a Beta  
distribution with parameters $(a,b)$, each evaluated at $p_{ri}$.
To simplify the analysis, we reparametrize  the
$b(p_{ri}; a, b)$ parameters by $\psi= a+b$  and
$\mu=a/(a+b)$. We assume a prior distribution on the $X_i$'s in the
form of~\eqref{eq:Ising} with homogeneous $\beta_{ij} \equiv \beta$
and a second-order neighborhood structure~\citep{li09} of $k=8$
neighbors for each interior pixel. We consider a standard uniform
prior density for $\mu$ and a $\operatorname{Gamma}( \zeta, \theta )$
prior density for the parameter $\psi$. Specifically, the prior
density for $\psi$ is $\operatorname{gamma}(\psi; \zeta, \theta )
\propto \psi^{\zeta -1} \exp( -\theta \psi)$. We assume uniform
hyperprior densities for $\alpha$ and $\beta$. The posterior density
of $\Theta = \{x_1,\ldots,x_n,\alpha,\beta,\psi,\mu\}$ is given by
\begin{multline*}
  \displaystyle\prod_{i=1}^n  \displaystyle\prod_{r=1}^R \bigl\{ b(p_{ri}; \mu\psi, \psi-\mu\psi)\bigr\}^{x_i} \\
\times  \tfrac{1}{Z(\alpha;\beta)}
\exp\biggl\{  -\theta \psi + \alpha \sum_{i} x_i 
 - \displaystyle\sum_{i \sim j} \beta (1 - \delta_{ij})\biggr\} \psi^{\zeta
  -1} \mathbf{1}_{[0 < \mu < 1]},
\end{multline*}
where for any set $S$, $\mathbf{1}_{S}$ denotes the indicator function
associated with $S$. Analytical inference being impractical to implement,
we derive a Metropolis-Hastings algorithm to estimate the posterior
densities of interest. Sampling from the above needs values of
$Z(\alpha,\beta)$ for which approaches typically involve, among
other strategies, offline estimation of the normalizing constant
through tedious MCMC methods at some values and then interpolation at
others~(for example, \citep{Maitra-Besag-1998}). Our approximations
  obviate the need for this offline approach and allow for the
  possibility of a direct approach. We now provide the MCMC framework for each parameter in $\Theta$, after
  introducing  additional notation for %denote $\Theta_{-\eta}$ to
%denote the set of all model parameters except $\eta$, that is
$\Theta_{-\eta} \equiv \Theta \setminus \{\eta\}$. 
 
\subsection{Posterior densities for MCMC simulations}
\label{sec:post:densities}
  \begin{enumerate}
\item {\bf The parameter $x_i$'s}: Let $x_{(-i)}=\{x_1, \ldots,  x_n\}\setminus \{x _i \}$. We propose to update  $x_i\in \{0, 1\}$
  via Gibbs' sampling. The full conditional of the posterior
  distribution of $x_i$, $p(x_i\mid x_{(-i)},\Theta_{-x},p)$ is proportional to
\begin{multline*}
  \biggl\{ \bigl(
    C_B\bigr)^R  \prod_{r=1}^R  p_{ri}^{\mu\psi} (1
    -p_{ri})^{(1-\mu)\psi} \biggr\}^{x_i} \\
\times   \exp\{ \alpha x_i - \beta \sum_{j\sim i} (1 -\delta_{ij}) \},
\end{multline*}
with
$C_B = \Gamma(\psi)/ \{ \Gamma(\mu\psi) \Gamma((1-\mu)\psi)\}$.
Let $A_i = \alpha + (\mu\psi -1) \sum_{r=1}^R \log p_{ri} + \{(1-\mu)\psi -1\}
\sum_{r=1}^R \log ( 1- p_{ri}) + R\log C_B.$
Then $\sum_{r=1}^R \log p_{ri}$ is
the same as $R\log \check p_i$ where  $\check p_i$ is the  harmonic mean of
$\{p_{ri}:r=1,2,\ldots,R\}$. Also, $\sum_{r=1}^R \log ( 1-
p_{ri})/R\equiv  \log\check q_i$  where $\check q_i$ is the harmonic mean of
$\{1-p_{ri}:r=1,2,\ldots,R\}$. Then 
$A_i \equiv \alpha + (\mu\psi -1) R \log( \check{p}_i ) + \{(1-\mu)\psi -1\}
R \log( \check{q}_i )  + R\log C_B$
%Note that when $x_i=1$, one has $\delta_{ij} = x_j$, and when
%$x_i=0$, one has $\delta_{ij}= 1 - x_j$ 
and 
\begin{multline*}
\operatorname{Pr}( X_i= 1 | x_{(-i)},\Theta_{-x},p) \propto \\
%\tfrac{ \exp\{ A_i - \beta \sum_{j\sim i} (1 - x_{j}) \} } {\exp\{ A_i
%- \beta \sum_{j\sim i} (1 - x_{j}) \} + \exp( - \beta \sum_{j\sim i} x_{j} ) } \\
%= \tfrac{ \exp\{ A_i - \sum_{j\sim i}\beta   + \beta \sum_{j\sim i}
%x_{j}  \}} {\exp\{ A_i  - \sum_{j\sim i}\beta   + \beta \sum_{j\sim
%i} x_{j} \} + \exp\{ - (\beta \sum_{j\sim i} x_{j} ) \} } \\
\tfrac{ \exp( A_i - \sum_{j\sim i}\beta) }
{\exp( A_i  - \sum_{j\sim i}\beta     )
+ \exp\{ - 2(\beta \sum_{j\sim i} x_{j}) \}  }
\end{multline*}


\item {\bf The parameter  $\beta$:} We have
$f( \beta | \Theta_{-\beta}, p) \propto { \exp\{ - \beta \sum_{i \sim j} (1 -\delta_{ij}) \} }/{Z( \alpha, \beta)}$,
  where $Z( \alpha, \beta)$
  %is as in~\eqref{eq:Isingconst} and
  will be
approximated numerically 
by $\tilde{Z}_\phi( \alpha, \beta)$ as defined in Section~\ref{sec:normal:approx}.
%per our
%Proposition~\ref{theo:Z}.
We let $\ddot\beta\sim$Gamma$(a,b)$ as our proposed update to $\beta$ with
$a/b = \beta$, and $a /b^2 = \gamma$, for some moderate $\gamma>0$
(e.g., $\gamma = 1$).  %That is, $b= \beta/\gamma$ and $a= \beta^2 / \gamma$.
This yields the \citet{hastings70} acceptance ratio that is the
minimum of 1 and 
\begin{multline*}
\tfrac{\tilde Z_\phi(\alpha,\beta)}{\tilde Z_\phi(\alpha,\ddot\beta)}
\tfrac{\Gamma ({\beta^2}/{\gamma})}{\Gamma({\ddot\beta^2}/{\gamma} )} 
\exp\biggl\{ -(\ddot\beta - \beta) \sum_{i\sim j} (1 - \delta_{ij})  \\
+ \frac1\gamma( \ddot\beta^2 - \beta^2)
\log(\beta\ddot\beta/\gamma)  \biggr\}.
\end{multline*}
%which, upon applying \citet{stirling1730}'s approximation for $\Gamma(z+1)$ simplifies to the minimum of 1 and 
\begin{comment}
\begin{align*} 
\tfrac{\Gamma({\beta^2}/\gamma)}{\Gamma( \ddot\beta^2/\gamma)} 
& \approx
\biggl( \tfrac{\beta_s'}{\beta_s}\biggr)
\exp\biggl(
\tfrac{\beta_s^2}{\gamma_s} \log\tfrac{\beta_s^2}{\gamma_s} - 
\tfrac{(\beta_s')^2}{\gamma_s} \log\tfrac{(\beta_s')^2}{\gamma_s}
+ (\tfrac{(\beta_s')^2}{\gamma_s} - \tfrac{\beta_s^2}{\gamma_s}) 
\biggr).
\end{align*}
Plugging in this last expression in the above \citet{hastings70} ratio, we obtain
\end{comment}
\begin{comment}
\begin{equation*}
\tfrac{\tilde Z_\phi(\alpha,\beta)}{\tilde Z_\phi(\alpha,\ddot\beta)}
\tfrac{\ddot\beta}{\beta}
\exp\bigl\{
\tfrac{\beta^2 + \ddot\beta^2}{\gamma}\log\tfrac{\beta}{\ddot\beta} 
+ \tfrac{\ddot\beta^2 - \beta^2}{\gamma}  
- ( \ddot\beta - \beta)\sum_{i\sim j} (1 - \delta_{ij})
\bigr\},
\end{equation*}
\end{comment}
\item {\bf The parameter  $\alpha$:} The full conditional for $\alpha$
  is given by
\[f( \alpha | \Theta_{-\alpha}, p) \propto
 \exp(  \alpha \sum_{i=1}^n x_{i} )/ Z( \alpha, \beta)\].
 Our proposed update to $\alpha$ is $\ddot\alpha\sim
N(\alpha, \sigma_\alpha^2)$ with a moderate $\sigma^2_\alpha$, (e.g.,
$\sigma^2_a = 1$), which, after incorporating the approximation in
Section~\ref{sec:normal:approx}.
%Proposition~\ref{theo:Z},
is accepted in a~\citep{metropolisetal53}
step with probability given by
%\begin{equation*}
$\min\left\{1,
{\tilde Z_\phi(\alpha,\beta)}\exp\{ (\ddot\alpha - \alpha) \sum_{i=1}^n x_{i} \} /{\tilde Z_\phi(\ddot\alpha,\beta)}\right\}$.
%\end{equation*}

\item {\bf The parameter  $\psi$:} The full conditional for $\psi$ is given by
  \begin{multline*}
  f( \psi | \Theta_{-\psi}, p ) \propto 
\biggl[ \tfrac{\Gamma(\psi)}{ \Gamma(\mu\psi) \Gamma([1-\mu]\psi)}
  \biggr]^{R \sum_{i}\! x_i} \\
\times \psi^{\zeta - 1} \exp[ \psi \{ \mu\log
  A + (1-\mu) \log B  - \theta \} ],
\end{multline*}
where $A= \prod_{i=1}^n \check{p}_i^{R x_i}$,
and $B = \prod_{i=1}^n \check{q}_i^{R x_i}$.
Using \citet{stirling1730}'s approximation to the factorial function,
the right-hand-side of the above equation can be approximated by
%%\begin{align*}
%${\Gamma(\psi)}/\{ \Gamma(\mu\psi) \Gamma((1-\mu)\psi) \}
%%& 
%\approx
%%\tfrac{1}{\sqrt{2\pi}} \tfrac{\psi^{\psi -0.5}}{(\mu\psi)^{\mu\psi -
%%0.5} ((1-\mu)\psi)^{(1-\mu)\psi -0.5}} \\ &=
%{1}/{\sqrt{2\pi}} [\psi^{1/2}/ \{ \mu^{\mu\psi - 0.5} (1-\mu)^{(1-\mu)\psi -0.5} \} ].$
%%\end{align*}
%%This  %expression suggests using a Gamma update for $\psi$. In fact,
%%this last
%%approximation yields
%Therefore,
\begin{multline}
%f( \psi | \Theta_{-\psi}, p ) \approx\propto
  \psi^{\frac{1}{2}n_1 + \zeta -1} \! \exp\biggl[  -\psi \{ \theta + \operatorname{Ent}(\mu) \\
    - \mu\log A - (1-\mu) \log B  \} \biggr],
\label{eq:psi}
\end{multline}
where $n_1= R \sum_{i=1}^n x_i$, and 
 $\operatorname{Ent}(\mu)= \mu \log \mu + (1-\mu) \log(1-\mu)$ is the negative of the entropy associated with the probabilities
$(\mu,  1 -\mu)$.
%This allows us to propose 
We update $\psi$ with the proposal
$\ddot\psi\sim$Gamma$( \tfrac{1}{2}n_1 + \zeta,
\theta + \operatorname{Ent}(\mu) - \mu\log A - (1-\mu) \log B ).$ 
%to update $\psi$. 
More generally, we can reduce this updating step to a Gibbs'
sampling step using the above approximated full conditional. 
The acceptance probability for $\ddot\psi$ is the minimum of 1 and 
\begin{multline*}
  \left(\tfrac{\Gamma(\ddot\psi)\, \Gamma(\mu\psi) \Gamma((1-\mu)\psi)}
       {\Gamma(\mu\ddot\psi) \Gamma((1-\mu)\ddot\psi)\,
            \Gamma(\psi)} \right)^{R \sum_{i}\! x_i}  \biggl(\tfrac{\psi}{\ddot\psi}\biggr)^{\frac{1}{2}n_1 + \zeta -1} \\
\times  \biggl(\tfrac{\ddot\psi}{\psi}\biggr)^{\zeta - 1} \!\!\!\!
\exp\bigl\{ (\ddot\psi -\psi)( \mu\log A + (1-\mu) \log B  - \theta ) \bigr\} \biggr. \\
\exp\bigl[ -  \{ \theta - \operatorname{Ent}(\mu) - \mu\log A -
(1-\mu) \log B  \} (\psi - \ddot\psi) \bigr],
\end{multline*}
which using~\eqref{eq:psi} yields the approximated acceptance ratio 
$
\min\{1, 
\exp[ (\psi - \ddot\psi) n_1 \{ \mu \log\mu + (1-\mu) \log( 1 - \mu)
\} ] \}$,
which is 1 whenever $\ddot\psi > \psi$ and so proposals $\ddot\psi >
\psi$ are always accepted. 



\item {\bf The parameter  $\mu$:} Here, we use a random walk update
  $\ddot\mu \sim \operatorname{U}(0,1)$. This yields the 
  Metropolis-Hastings acceptance ratio that is the minimum of 1 and 
\begin{multline*}
\biggl(\tfrac{\Gamma(\psi)}{\Gamma(\ddot\mu\psi) \Gamma((1-\ddot\mu)\psi)}
\tfrac{\Gamma(\mu\psi) \Gamma((1-\mu)\psi)}{\Gamma(\psi)} \biggr)^{n_1} \, \\
\times  
\exp\biggl\{ \psi \ddot\mu \log A + \psi (1 -\ddot\mu) \log B \\
- \psi \mu \log A - \psi (1-\mu)  \log B \biggr\}.
%\\
%\end{multline*}
%Using Stirlings approximation, one gets the approximative ratio
%\begin{multline*}
%\min\biggl\{1, \exp\biggl\{ n_1\biggl( \psi [\mu \log \mu + (1-\mu) \log(1-\mu)]  - 0.5 \log[ \mu(1-\mu) ] \\
%\biggl.  - \psi [\ddot\mu \log \ddot\mu + (1-\ddot\mu) \log(1-\ddot\mu)]    + 0.5 \log[ \ddot\mu(1-\ddot\mu) ] \biggr) \biggr\}  \exp\{ \psi (\ddot\mu -\mu) ( \log A - \log B) \} \biggr\} \\
%\approx
%\exp\biggl\{ \psi (\ddot\mu -\mu) \log (A/B) + \psi n_1 ( \operatorname{Ent}(\mu) -  \operatorname{Ent}(\ddot\mu) )\\
% + \tfrac{n_1}{2} \log \biggl(\tfrac{\ddot\mu(1-\ddot\mu)}{\mu(1-\mu)}\biggr) \biggr\},
\end{multline*}
%where the last approximation follows by applying
%\citet{stirling1730}'s approximation to the ratios of the $\Gamma()$ functions.
%%where $\operatorname{Ent}(\mu)= \mu \log \mu + (1-\mu) \log(1-\mu)$ is the negative of the entropy associated with the probabilities
%%$(\mu, \, 1 -\mu)$.
\end{enumerate}
\subsection{Results}
The above posterior densities were used in the context of activation
detection in the fMRI dataset. For this example, we set the
hyperprior
parameters $\theta=1$ and $\zeta = 10$. This reflects our general
a priori view that $\psi= a + b$ is large. We initialized our MCMC
simulations with $(\alpha,\beta,\psi,\mu) = (0.001, 0.0025, 1,
0.001)$ and used collected a sample size of 
10,000 realization after a burn-in period of the same number of iterations.
The vertex values (for the autologistic variables) were updated (and 
initialized after a burn-in period of 3,000 iterations)
with the \citet{Swendsen-Wang-1987} algorithm or the single-site
updating given in point (1) of Section~\ref{sec:post:densities} above. 
The posterior 
probability of activation, that is,  the estimated posterior means of
the $x_i$s at each voxel, are displayed in Figure~\ref{fig1}. 
As is
customary in fMRI, the image is displayed using a radiological
view. Thus, the right-hand side of the brain is imaged as the
left-hand side.
\begin{figure}[h]
  \begin{center}
    % The arguments in the next line are {height}{optional width}{used
    % only by OUP for typesetting}[filename, in directory art]
    \mbox{\subfigure[]{\includegraphics[width=0.166\textwidth]{righthand20thslice-k8-normalSW-crop}}
          \subfigure[]{\includegraphics[width=0.166\textwidth]{righthand20thslice-k8-normalSU-crop}}
    % note that files may not be rotated
          \subfigure[]{\includegraphics[width=0.166\textwidth]{righthand20thslice-CT2-crop}}}
  \end{center}
  \caption{Leftmost and middle panels: the posterior probabilities of activation in the fMRI
    experiment using (a) Swendsen-Wang and (b) single-site
    updating. Rightmost panel (c): p-values
after cluster-wise thresholding for p-values $< 0.001$.
 Displays are in radiological view in the log scale.} 
  \label{fig1}
\end{figure}
In the figure, we only display posterior probabilities that are
greater than 0.5. 
It is clear that the
 posterior probabilities of
activation using either Swendsen-Wang or single-site updating are essentially
indistinguishable.
For comparison, we have provided the results obtained upon using the commonly-used cluster-wise thresholding of the $p$-values of the test statistic. Here, activation regions are detected by drawing clusters of connected components each containing a pre-specified
number of voxels with $p$-values below a specified threshold~\citep{fristonetal94,hayasakaandnichols03}.  
To obtain our activation map,
we choose a 2-D second-order neighborhood, 
a threshold of 0.001  for the $p$-values, 
following the recommendations of \citet{wooetal14}, 
and a minimum cluster size of 4 pixels, as optimally recommended by \citet{fromanetal95} using the AFNI software~\citep{cox96,coxandhyde97,cox12}.
Although a detailed analysis of the results is
beyond the purview of this paper, we note from the Bayesian model
that there is very high
posterior probability of activation in the left primary motor 
(M1) and pre-motor (pre-M1) cortices and the supplementary motor
areas. There are also some areas on the right with high posterior
probability of activation, perhaps as a consequence of the left-hand
finger-tapping experiment that was also a part of the larger
experiment. 
While the activation maps using cluster-wise thresholding are generally similar to those obtained using Bayesian inference, there are many stray pixels determined to be activated. Moreover, unlike cluster-wise thresholding, Bayesian methods provide us with the posterior probability of activation and this can be used in informing further decisions.



==> inequality.tex <==
For any given $\epsilon >0$, we have
\begin{multline}
\operatorname{pr}(  \bigl| Z(\alpha, \beta) - Z( \alpha, \beta | {\cal G}_{n.m} )
\bigr|
> \epsilon Z( \alpha, \beta | {\cal G}_{n.m} ) ) = \\
\operatorname{pr}(   Z(\alpha, \beta) - Z( \alpha, \beta | {\cal G}_{n.m} )
> \epsilon Z( \alpha, \beta | {\cal G}_{n.m} ) ) 
+ \operatorname{pr}(   Z(\alpha, \beta) - Z( \alpha, \beta | {\cal G}_{n.m} )
< -\epsilon Z( \alpha, \beta | {\cal G}_{n.m} ) ).
\label{eq:pr:bound:Z:1}
\end{multline}
Let $\ell_m = \min\{ \ell_2, m\}.$ 
We have
\begin{multline}
\operatorname{pr}(   Z(\alpha, \beta) - Z( \alpha, \beta | {\cal G}_{n.m} )
> \epsilon Z( \alpha, \beta | {\cal G}_{n.m} ) ) 
= \\
\operatorname{pr}\bigl[  \sum_{\ell=1}^{n-1}\binom{n}{\ell} 
\sum_{s=0}^{\ell_m}
\{ \hat{p}(s|\ell) - (1 + \epsilon)p(s|\ell) \} \exp(\alpha'\ell + 2 \beta s) > 0 \bigr] \leq \\
\operatorname{pr}\bigl(  \cup_{\ell=1}^{n-1}
\biggl[ \sum_{s=0}^{\ell_m}
( Y(s,\ell) - (1 + \epsilon)\binom{n}{\ell}p(s|\ell) ) \exp( 2 \beta s) > 0 \biggl] \bigr)
\leq \\
 \sum_{\ell=1}^{n-1} 
\operatorname{pr}\bigl\{ \sum_{s=0}^{\ell_m}
( Y(s,\ell) - (1 + \epsilon)\binom{n}{\ell}p(s|\ell) ) \exp( 2 \beta s) > 0 
\bigr\}.
\label{eq:pr:bound:Z:2}
\end{multline}
Let $Z_{\ell} = \sum_{s=0}^{\ell_m} ( Y(s,\ell) - \binom{n}{\ell}p(s|\ell) ) \exp( 2 \beta s), $ and for every real number $u$ consider
${\cal M}_{\ell}(u) =  \sum_{s=0}^{\ell_m} p(s|\ell) \exp( u s),$
the moment generating function associated
with the hypergeometric distribution with probabilities given by $\{p(\cdot|\ell)\}$ evaluate at $u$.
For $\delta > 0$, consider the event 
$A_{\ell, \delta} = \{  Z_{\ell}^2 \leq \delta^2 \binom{n}{\ell}^{2\kappa} {\cal M}_{\ell}(4\beta) \},$ 
and its complement $ A_{\delta,\ell}^{c}$, for some
$1/2 < \kappa < 1$.
We have
\begin{multline*}
\operatorname{pr}\bigl\{ \sum_{s=0}^{\ell_m}
( Y(s,\ell) - (1 + \epsilon)\binom{n}{\ell}p(s|\ell) ) \exp( 2 \beta s) > 0 
\bigr\}  = \\
\operatorname{pr}\bigl\{ Z_{\ell} > \epsilon \binom{n}{\ell} {\cal M}_{\ell}(2\beta)
 \text{\ and \ } A_{\delta,\ell} \bigr\}
+  \operatorname{pr}\bigl\{ 
Z_{\ell} > \epsilon \binom{n}{\ell} {\cal M}_{\ell}(2\beta)
 \text{\ and \ } A_{\delta,\ell}^{c} \bigr\}.
\end{multline*}
By Chebychev's inequality, 
\begin{multline*}
 \operatorname{pr}\bigl\{ 
Z_{\ell} > \epsilon \binom{n}{\ell} {\cal M}_{\ell}(2\beta)
 \text{\ and \ } A_{\delta,\ell}^{c} \bigr\}
\leq \operatorname{pr}( A_{\delta,\ell}^{c} )
\leq \operatorname{Var}(Z_{\ell}) / (\delta^2 \binom{n}{\ell}^{2\kappa} {\cal M}_{\ell}(4\beta) ).
\end{multline*}
Note that the variables $\{Y(s,\ell)\}_s$ are jointly multinomial.
So 
\begin{align*}
 \operatorname{Var}(Z_{\ell}) 
& = \binom{n}{\ell} \biggl[ \sum_{s=0}^{\ell_m}  p(s|\ell)(1 - p(s|\ell)) \exp(4 \beta s)
- 2 \sum_{s=1}^{\ell_m -1} \sum_{t=0}^s p(s|\ell)p(t|\ell) \exp\{2\beta(s+t)\} \biggr] \\
& \leq \binom{n}{\ell}  \sum_{s=0}^{\ell_m} p(s|\ell)(1-p(s|\ell))\exp( 4\beta s )
\leq \binom{n}{\ell}  {\cal M}_{\ell}(4\beta).
\end{align*}
Therefore
$ \operatorname{pr}\bigl\{ 
Z_{\ell} > \epsilon E_{\ell}
 \text{\ and \ } A_{\delta,\ell}^{c} \bigr\}
\leq  \binom{n}{\ell}^{1 - 2\kappa} /\delta^2.$
Note that
$\binom{n}{\ell} = \prod_{i=1}^{\ell}[ \{ (n+1)/i\} - 1].$
Consequently, $n \leq \binom{n}{\ell} \leq \binom{n}{n/2}$ for 
$\ell \in \{1, \ldots, n-1\}$.
Also, as $1- 2\kappa < 0$,
the above probability goes to zero 
uniformly on $\ell$ as $n$ increases.

To bound from above $\operatorname{pr}\bigl\{ Z_{\ell} > \epsilon \binom{n}{\ell} {\cal M}_{\ell}(2\beta)  \text{\ and \ } A_{\delta,\ell} \bigr\}$,
we use the bounded difference inequality of \cite{vandergeer-inequalities}.
This yields
\begin{align*}
\operatorname{pr}\bigl\{ Z_{\ell} > \epsilon \binom{n}{\ell} {\cal M}_{\ell}(2\beta)  \text{\ and \ } A_{\delta,\ell} \bigr\}
& \leq \exp\bigl( - \frac{2 \epsilon^2 \binom{n}{\ell}^2 ({\cal M}_{\ell}(2\beta) )^2}
{\delta^2 \binom{n}{\ell}^{2\kappa}  {\cal M}_{\ell}(4\beta) } \bigr) \\
& = \exp \bigl\{ - \bigl( \frac{\epsilon}{\delta}\bigr)^2
 \binom{n}{\ell}^{2(1- \kappa)} \frac{({\cal M}_{\ell}(2\beta) )^2}{ {\cal M}_{\ell}(4\beta) }
\bigr\} \\
& \leq \exp \bigl\{ - n\, \bigl( \frac{\epsilon}{\delta}\bigr)^2 C(\beta, k)\bigr\},
\end{align*}
where $C(\beta, k)$ is a positive constant independent of $n$ and $\ell$.
This constant can be obtained from the following argument.
%First let $\ell_2 = \ell(\ell-1)/2$, and $n_2= n(n-1)/2$.
We have
\begin{align*}
p(s|\ell) & = \binom{m}{s} \prod_{i=0}^{m -s-1} (n_2 - \ell_2 - i)\prod_{i=0}^{\ell_2 -1}
(\ell_2 - i) / \bigl( \prod_{i=0}^{\ell_2 -s -1} ( \ell_2 -s - i) \prod_{i=0}^{m -1}
( n_2 - i) \bigr) \\
&= \binom{m}{s} \prod_{i=0}^{m -s-1} (n_2 - \ell_2 - i)\prod_{i=0}^{s -1}
(\ell_2 - i) / \prod_{i=0}^{m -1} ( n_2 - i) \\
&= \binom{m}{s} \prod_{i=0}^{m -s-1} (1 - \frac{\ell_2 + i}{n_2})\prod_{i=0}^{s -1}
(\frac{\ell_2}{n_2} - \frac{i}{n_2}) / \prod_{i=0}^{m -1} ( 1 -\frac{i}{n_2} ).
\end{align*}
Therefore,
\begin{align*}
p(s|\ell) & \leq \binom{m}{s} \bigl(1 - \frac{\ell_2}{n_2}\bigr)^{m - s} \bigl(\frac{\ell_2}{n_2}\bigr)^{s} / \bigl( 1 - \frac{m-1}{n_2}\bigr)^{m}, \\
p(s|\ell) & \geq \binom{m}{s}  \bigl(1 - \frac{\ell_2 + m - s - 1}{n_2}\bigr)^{m - s} \bigl(\frac{\ell_2 - s  + 1}{n_2}\bigr)^{s} \\
& \geq \binom{m}{s}  \bigl(1 - \frac{\ell_2 + m -s_{min} - 1}{n_2}\bigr)^{m - s} \bigl(\frac{\ell_2 - \ell_m  + 1}{n_2}\bigr)^{s},
\end{align*}
where $s_{min} = \max \{ 0, m - n_2 + \ell_2\}$.
Consequently,
\begin{align*}
{\cal M}_{\ell}(4\beta) & \leq 
 \sum_{s=0}^{m} \binom{m}{s} \bigl(1 - \frac{\ell_2}{n_2}\bigr)^{m - s} \bigl(\frac{\ell_2}{n_2}\bigr)^{s} \exp(4\beta s)  /\bigl( 1 - \frac{m-1}{n_2}\bigr)^{m},\\
{\cal M}_{\ell}(2\beta) & \geq
 \sum_{s=s_{min}}^{\ell_m} \binom{m}{s} \bigl(1 - \frac{\ell_2 + m -s_{min} - 1}{n_2}\bigr)^{m - s} \bigl(\frac{\ell_2 - \ell_m + 1}{n_2}\bigr)^{s} \exp(2\beta s).
 \end{align*}
The numerator in the first expression is the moment generating function of a binomial distribution
with probability of success $\ell_2/n_2$ and $m$ trials evaluated at $4\beta$. So 
${\cal M}_{\ell}(4\beta) \leq \{ 1 + \frac{\ell_2}{n_2}( \exp(4\beta) -1 ) \}^{m} / \bigl( 1 - \frac{m-1}{n_2}\bigr)^{m}.$
Similarly, using now the binomial theorem, we also get for $\ell_m \leq n_2 - m$, 
${\cal M}_{\ell}(2\beta) \geq \{ 1 - \frac{\ell_2+m -1}{n_2}
+\frac{\ell_2 -m+1}{n_2} e^{2\beta} \}^{m}.$




==> pistachioapp.tex <==
\subsection{The pistachios images}
\label{sec:pistachios}
Two tests were run: the first one considers the order one neighborhood. It consists of testing
$H_0: \beta_p = \beta_v$ against $H_1: \beta_p \not= \beta_v$.
The second test consider the order two neighborhood where $\beta_p$  is the parameter associated with the order one neighborhood, and $\beta_v$ is the parameter associated with the remaining neighbors of the second order neighborhood. This test consists of testing
$H_0: \beta_v = 0$ against $H_1: \beta_v \not= 0$.
The second test was only done if the first null is not rejected.
The $p$-values were computed from 1000 samples generated from the null and using the
parameters associated with the null on the corresponding image.
\begin{table}
  \begin{center}
  \caption{Paremeter estimates for the pistachios images.
    The first test (column 5) corresponds to the test for first order isotropic model against a first order anisotropic model.
    The second test (column 6) corresponds to the test for first order isotropic model against a
    second order anisotropic model.}
    \label{table:pistachio-tests}
    \begin{tabular}{c|clc|cc} \\
          &   \multicolumn{3}{c}{Parameters}    &  $H_o: \beta_p = \beta_v$   & $H_o : \beta_v = 0$ \\     
   Image  &  $\alpha$    &  $\beta_p$  & $\beta_v$ & $p$-value &  $p$-value \\ \hline
   I      &    0.41   &  0.35    & 0.35   & 1.00           &  0.48 \\
   II     &    0.02   &  0.0001  & 2.22   & 0.008          &  -    \\
   III    &    0.06   &  0.68    & 0.68   & 0.58           &  0.24  \\   
   %  III    &   -0.01   &  0.66    & 0.66   & 1.00           &  0.80  \\
   IV     &    0.05   &  0.66    & 0.66   & 0.97           &  0.24  \\ \hline   
%   IV     &    0.07   &  0.65    & 0.65   & 0.96           &  0.61  \\ \hline
  \end{tabular}
\end{center}
\end{table}

   
 



==> proofA2.tex <==
For every pair of positive integers $h{<}g$, Stirling's
formula~\citep{stirling1730,demoivre1733} yields
\begin{equation}
\begin{split}
\begin{pmatrix} g \\ h \end{pmatrix} 
& = \tfrac{1}{\sqrt{2\pi}}  \tfrac{g^{g+\frac{1}{2}}}{ (g-h)^{g-h +
    \frac{1}{2}} h^{h + \frac{1}{2}}}\{ 1 + \omega(g, h)\}\\&= \tfrac{1}{\sqrt{2\pi g}} \bigl(1 - \tfrac{h}{g}\bigr)^{-g + h - \frac{1}{2}} 
    \bigl( \tfrac{h}{g}\bigr)^{-h - \frac{1}{2}} \{ 1 + \omega(g, h)\},
    \end{split}
    \label{eq:Stirling}
\end{equation}
where $\omega(g,h)$ denotes the error in Stirling's approximation.
Let $p{=} (\ell {-} 1)/(n{-}1)$. let $n_1 {=} n{-}1$, and $\bar{\theta} {=} 1 {-} \theta$.
Consider the first binomial term in the definition of $p_{d,m}(\cdot | \ell)$
Following the proof of the de-Moivre-Laplace's normal approximation
to the binomial distribution \citep{Pinsky},
write $r{=} n_1 p\theta {+} x \sqrt{n_1 p \theta \bar{\theta}}$. Using (\ref{eq:Stirling}),
we have, for values of $r {>} 0$ and $r {<} k$,
\begin{align*}
\begin{pmatrix} k \\ r \end{pmatrix} = & \begin{pmatrix} n_1 \theta \\  n_1 p \theta + x \sqrt{n_1 p \theta \bar{\theta}} \end{pmatrix} 
 =  ( 2\pi n_1 p\theta(1-p))^{-\frac{1}{2}}\,\\ &\times 
p^{-n_1p\theta - x\sqrt{n_1 p\theta\bar{\theta}}} (1
  -p)^{-n_1(1-p)\theta + x\sqrt{n_1 p \theta\bar{\theta}}} \\
&\times \{ 1 + \omega(k, r)\} 
 \bigl( 1 + \tfrac{x}{p} \sqrt{\tfrac{p\bar{\theta}}{n_1 \theta}} \bigr)^{-n_1 p\theta - x\sqrt{n_1 p\theta\bar{\theta}}}\\
& \times \bigl( 1 - \tfrac{x}{1-p} \sqrt{\tfrac{p \bar{\theta}}{n_1 \theta}} \bigr)^{-n_1 (1-p)\theta + x\sqrt{n_1 p \theta\bar{\theta}}}.
\end{align*}
For $\abs{z}{ <}
1$, we have $\log(1 {-}z ) {=} -z {-} z^2/2 {+} O( z^3)$ and $\log( 1 {+} z) {=} z {-} z^2/2 {+} O(z^3)$. With these identities, we have
\begin{comment}
\begin{equation*}
\begin{split}
  {-n_1 \theta (1\!\! - \!\! p)} &\log{\big(1 \!\! - \!
    \tfrac{x}{1-p}\sqrt{\tfrac{p\bar\theta}{n_1\theta}} 
  \big)}
%  \\
%& \qquad \qquad=
= x\sqrt{n_1 p \theta \bar{\theta}} \! +\! \tfrac{1}{2} \tfrac{px^2  \bar{\theta}}{1-p} \! + \! R_1(x), 
\end{split}
\end{equation*}
%and 
\begin{equation*}
\begin{split}
 \text{\hspace{-12pt} and\ } \qquad x\sqrt{n_1 p \theta\bar{\theta}} \log{\big(1 -
    \tfrac{x}{1-p}\sqrt{\tfrac{p\bar\theta}{n_1\theta}} 
  \big)} 
= -\tfrac{x^2 p \bar{\theta}}{1-p} + R_2(x),
\end{split}
\end{equation*}
where the errors $R_1(x)$ and $R_2(x)$ are of order $\epsilon_1(x)= {\cal O}( x^3 k^{-1/2} p^{3/2}(1-p)^{-2})$.
That is,
\end{comment}
\begin{multline}
\bigl( -n_1 \theta(1-p) + x\sqrt{n_1 p \theta\bar{\theta}} \bigr)   \log{\left(1 -
    \tfrac{x}{1-p}\sqrt{\tfrac{p\bar\theta}{n_1\theta}} 
  \right)} \\
 = x\sqrt{n_1 p \theta\bar{\theta}} -\tfrac{x^2}{2(1- p)} p\bar{\theta}
+ \epsilon_1(x),
\label{eq:Stirling:1}
\end{multline}
%Similarly,
where $\epsilon_1(x)= {\cal O}( x^3 k^{-1/2} p^{3/2}(1-p)^{-2})$, and
\begin{multline}
\bigl( -n_1 p\theta - x\sqrt{n_1 p \theta\bar{\theta}} \bigr)  \log\big(  1 + \tfrac{x}{p} 
\sqrt{\tfrac{p\bar{\theta}}{n_1 \theta}} \big) \\
= -x\sqrt{n_1 p \theta\bar{\theta}} -\tfrac{x^2}{2} \bar{\theta}  + \epsilon_2(x),
\label{eq:Stirling:2}
\end{multline}
where $\epsilon_2(x){=} {\cal O}( x^3/\sqrt{kp})$.
Combining \eqref{eq:Stirling:1} and \eqref{eq:Stirling:2} gives
$\begin{pmatrix} k \\ r \end{pmatrix} \approx$
\begin{equation*}
\begin{split}
%\begin{pmatrix} k \\ r \end{pmatrix} \approx \\ 
\tfrac{\exp\big\{ -\tfrac{x^2}{2(1 -p)} \bar{\theta} \big\} }
{\sqrt{2\pi n_1 p\theta (1-p)}} %\\
%& \times
p^{-n_1 p\theta - x\sqrt{n_1 p \theta\bar{\theta}}}  
 (1 -p)^{-n_1 (1-p)\theta + x\sqrt{n_1 p \theta\bar{\theta}}}
\end{split}
\end{equation*}
Similarly we get
$ \begin{pmatrix} n {-} 1 {-} k \\ \ell {-} 1{-} r \end{pmatrix}   {=}
\begin{pmatrix} n_1 \bar{\theta} \\ n_1 p \bar{\theta}  {-} x \sqrt{n_1 p \theta\bar{\theta}} \end{pmatrix} \approx $
\begin{equation*}
\begin{split}
%\binom{n {-} 1 {-} k}{\ell {-} 1{-} r}  & {=} \binom{n_1 \bar{\theta}}{ n_1 p \bar{\theta}  {-} x \sqrt{n_1 p \theta\bar{\theta}} } \\
% & \approx
\tfrac{ \exp\big\{ -\tfrac{x^2}{2(1 -p)} \theta \big\} }{ \sqrt{2\pi n_1 p \bar{\theta}(1{-}p)}}
p^{-n_1 p \bar{\theta} + x\sqrt{n_1 p \theta\bar{\theta}}}
% \\ &\qquad \times
(1{-}p)^{-n_1 (1-p)\bar{\theta} - x\sqrt{n_1 p \theta\bar{\theta}}},
\end{split}
\end{equation*}
\begin{equation*}
\mbox{\hspace{-3.5cm} and }\quad \begin{pmatrix} n {-} 1 \\ \ell {-} 1\end{pmatrix}  \approx
\tfrac{ (1 -p)^{-n_1(1-p)} p^{-n_1p}}{\sqrt{ 2\pi n_1 p (1- p) }}.
\end{equation*}
%
%\begin{equation*}
%\mbox{\hspace{-2.9cm} Further, } \quad p_{d,m}(r | \ell)  \approx  % \big( 2\pi n_1 p (1-p) \theta \bar{\theta} \big)^{-\frac{1}{2}} \exp\big( -{x^2}/ (2(1 -p) ) \big) \\
%=
%\tfrac{\exp\big( -\tfrac{ (r-n_1p\theta)^2}{ 2 n_1 p (1-p) \theta\bar\theta} \big)}{ \sqrt{2\pi n_1 p (1-p) \theta\bar\theta} }.
%\end{equation*}
 Further, $p_{d,m}(r | \ell)  \approx \tfrac{\exp\big( -\tfrac{ (r-n_1p\theta)^2}{ 2 n_1 p (1-p) \theta\bar\theta} \big)}{ \sqrt{2\pi n_1 p (1-p) \theta\bar\theta} },$
with the approximation being valid provided that
$\{|x| /(1-p)\} \sqrt{p\bar{\theta}/k} < 1$ and $(|x|/p)\sqrt{p 
\bar{\theta}/k} < 1$. That is,
$|x| < \sqrt{k/\bar{\theta}} \min\{ \sqrt{p}, (1-p)/\sqrt{p}\}$.
If $\ell \in [ a n^{\delta}, n - an^{\delta}]$ for some constants
$a>0$, and $0< \delta < 1$,
then $\min_p   \min\{ \sqrt{p}, (1-p)/\sqrt{p}\} \geq (a n^{\delta} -1)/(n-1) = {\cal O}( n^{\delta -1}).$
In this case, 
$\epsilon_1(x) \leq (k/\bar{\theta})^{\frac{3}{2}} k^{-\frac{1}{2}} a n^{\delta-1} =
{\cal O}( n^{\delta -1})$, and
\[\epsilon_2(x) \leq (k/\bar{\theta})^{\frac{3}{2}} k^{-\frac{1}{2}} a^{3} n^{3(\delta -1)}
\sqrt{\tfrac{n-1}{a n^{\delta} -1}} = {\cal O}( n^{(\frac{5}{2})(\delta -1)} ).\]
For $\delta {=} 1/2$, $|x| {<} {\cal O}\bigl( [\theta/ \bar{\theta}]^{\frac{1}{2}} \bigr)$, and
$\epsilon_i(x) {\leq}  {\cal O}( n^{-\frac{1}{2}} ),$
$i=1,2$.

